Adversarial Preference Optimization: Enhancing Your Alignment via RM-LLM Game

Human preference alignment is essential to improve the interaction quality of large language models (LLMs). Existing alignment methods depend on manually annotated preference data to guide the LLM optimization directions. However, continuously updating LLMs for alignment raises a distribution gap between model-generated samples and human-annotated responses, hindering training effectiveness. To mitigate this issue, previous methods require additional preference annotation on newly generated samples to adapt to the shifted distribution, which consumes a large amount of annotation resources. Targeting more efficient human preference optimization, we propose an Adversarial Preference Optimization (APO) framework, in which the LLM and the reward model update alternatively via a min-max game. Through adversarial training, the reward model can adapt to the shifted generation distribution of the LLM without any additional annotation. With comprehensive experiments, we find the proposed adversarial training framework further enhances existing alignment baselines in terms of LLM helpfulness and harmlessness. The code is at https://github.com/Linear95/APO.

==> tables/data_preparation_1.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{r|l|l|l}
\toprule
      & \multicolumn{2}{l|}{\textbf{H\&H Training Set} (91K)} & \multicolumn{1}{l}{\textbf{H\&H Testing Set} (4.7K)} \\
\hline
\multicolumn{1}{r|}{Preference Data Pairs} & \multicolumn{2}{l|}{Testing RM Training} & \multicolumn{1}{l}{Testing RM Evaluation} \\
%\midrule
\hline
      & \textbf{H\&H RM Training Set} (20K) & \multicolumn{1}{l|}{\textbf{H\&H LLM Training Set} (71K)} & \multicolumn{1}{l}{ \textbf{H\&H Testing Set} (4.7K)} \\
\hline
Preference Data Pairs& Baseline RM Training &  -      & \multicolumn{1}{l}{Baseline RM Evaluation} \\
\hline
Instruction Queries &   APO RM Training   & LLM Rejection Sampling and Training &  LLM Agent Evaluation \\
\hline
GPT-4 Golden Answers & APO RM Training &    -   &  APO RM Evaluation \\
\bottomrule
\end{tabular}%
}
    \caption{Data preparation and usage. The original  H\&H training set is used to learn a testing RM to automatically evaluate the quality of LLM responses.
    %Next, we split H\&H training set into an RM training set and an LLM training set.
    The split H\&H RM training set is for baseline RM and APO RM training. Queries in the H\&H LLM training set are utilized to update the LLM agent. Both RM and LLM's performance are evaluated on the  H\&H testing set.  
 }
    \label{tab:data_preparation}
\end{table}


==> tables/llm_results.tex <==
\begin{table*}[t]
\centering
 \caption{Training setups and performance of LLM agents during the rejection sampling process.}
    \label{tab:llm_results}   
    \vspace{-1mm}
  % Table generated by Excel2LaTeX from sheet 'APO_final'
  \resizebox{0.995\textwidth}{!}{
\begin{tabular}{llllrrr}
\toprule
\textbf{Round}       & \textbf{Model} & \textbf{Base} & {\textbf{Rejection Sampling RM}} & \textbf{LR} & \textbf{Avg. RM$_\text{All}$  Score} & \textbf{ Avg. RM$_\text{Test}$  Score} \\
\midrule
 Rnd. 0 & Alpaca & Alpaca & {-}      &   -    & 1.246 & 0.922 \\
  \midrule
 Rnd. 1 & LLM$_\text{RJS}$-v1 & Alpaca & {RM$_\text{Base}$} & 5e-6 &        1.546 & 1.204 \\
Rnd. 1 & LLM$_\text{APO}$-v1 & Alpaca & {RM$_\text{APO}$-v1} & 5e-6 &     1.610 & 1.251 \\
Rnd. 1 & LLM$_\text{RJS}$-AB & Alpaca & {RM$_\text{Base}$-AB} & 5e-6 &     1.534 & 0.959 \\
\midrule
Rnd. 2 & LLM$_\text{RJS}$-v2 & LLM$_\text{RJS}$-v1 & {RM$_\text{Base}$} & 2e-6 &    1.896 & 1.551 \\
Rnd. 2 & LLM$_\text{APO}$-v2seq & LLM$_\text{APO}$-v1 & {RM$_\text{APO}$-v2seq} &   2e-6   & 2.008 & 1.649 \\
Rnd. 2 & LLM$_\text{APO}$-v2 &  LLM$_\text{APO}$-v1 &      {RM$_\text{APO}$-v2}      &  2e-6     & 1.975 & 1.586 \\
\midrule
Rnd. 3 & LLM$_\text{RJS}$-v3 & LLM$_\text{RJS}$-v2 & {RM$_\text{Base}$} & 9e-7 &    2.106 & 1.764 \\
Rnd. 3 & LLM$_\text{APO}$-v3seq & LLM$_\text{APO}$-v2seq & {RM$_\text{APO}$-v3seq} &   9e-7   & 1.947 & 1.624 \\
Rnd. 3 & LLM$_\text{APO}$-v3 &  LLM$_\text{APO}$-v2 &      {RM$_\text{APO}$-v3}      &  9e-7     &\textbf{2.204} & \textbf{1.807} \\
\bottomrule
\end{tabular}%
}
   
\end{table*}

==> tables/llm_results_1113.tex <==
\begin{table}[t]
\centering
 \caption{Training setups and performance of LLM agents during the rejection sampling process.}
    \label{tab:llm_results}    
  % Table generated by Excel2LaTeX from sheet 'APO_final'
  \resizebox{\textwidth}{!}{
\begin{tabular}{llllrrrr}
\toprule
\textbf{Round}       & \textbf{Model} & \textbf{Base} & {\textbf{Scoring RM}} & \textbf{LR} & \textbf{RM$_\text{All}$ Score} & \textbf{ RM$_\text{Test}$ Score} & \textbf{GPT-4 Win Rate} \\
\midrule
 Rnd. 0 & Alpaca & Alpaca & {-}      &   -    & 1.246 & 0.922 \\
  \midrule
 Rnd. 1 & LLM$_\text{RJS}$-v1 & Alpaca & {RM$_\text{Base}$} & 5e-6 &        1.546 & 1.204 \\
Rnd. 1 & LLM$_\text{APO}$-v1 & Alpaca & {RM$_\text{APO}$-v1} & 5e-6 &     1.610 & 1.251 \\
\midrule
Rnd. 2 & LLM$_\text{RJS}$-v2 & LLM$_\text{RJS}$-v1 & {RM$_\text{Base}$} & 2e-6 &    1.896 & 1.551 \\
Rnd. 2 & LLM$_\text{APO}$-v2seq & LLM$_\text{APO}$-v1 & {RM$_\text{APO}$-v2seq} &   2e-6   & 2.008 & 1.649 \\
Rnd. 2 & LLM$_\text{APO}$-v2 &  LLM$_\text{APO}$-v1 &      {RM$_\text{APO}$-v2}      &  2e-6     & 1.975 & 1.586 \\
\midrule
Rnd. 3 & LLM$_\text{RJS}$-v3 & LLM$_\text{RJS}$-v2 & {RM$_\text{Base}$} & 9e-7 &    2.106 & 1.764 \\
Rnd. 3 & LLM$_\text{APO}$-v3seq & LLM$_\text{APO}$-v2seq & {RM$_\text{APO}$-v3seq} &   9e-7   & 1.947 & 1.624 \\
Rnd. 3 & LLM$_\text{APO}$-v3 &  LLM$_\text{APO}$-v2 &      {RM$_\text{APO}$-v3}      &  9e-7     & \textbf{2.204} & \textbf{1.807} \\
\bottomrule
\end{tabular}%
}
   
\end{table}

==> tables/llm_results_no_seq.tex <==
\begin{table}[t]
\centering
 \caption{Training setups and performance of LLM agents during the rejection sampling process.}
    \label{tab:llm_results}   
    \vspace{-1mm}
  % Table generated by Excel2LaTeX from sheet 'APO_final'
  \resizebox{0.995\textwidth}{!}{
\begin{tabular}{llllrrr}
\toprule
\textbf{Round}       & \textbf{Model} & \textbf{Base} & {\textbf{Rejection Sampling RM}} & \textbf{LR} & \textbf{Avg. RM$_\text{All}$  Score} & \textbf{ Avg. RM$_\text{Test}$  Score} \\
\midrule
 Rnd. 0 & Alpaca & Alpaca & {-}      &   -    & 1.246 & 0.922 \\
  \midrule
 Rnd. 1 & LLM$_\text{RJS}$-v1 & Alpaca & {RM$_\text{Base}$} & 5e-6 &        1.546 & 1.204 \\
Rnd. 1 & LLM$_\text{APO}$-v1 & Alpaca & {RM$_\text{APO}$-v1} & 5e-6 &     1.610 & 1.251 \\
Rnd. 1 & LLM$_\text{RJS}$-AB & Alpaca & {RM$_\text{Base}$-AB} & 5e-6 &     1.534 & 0.959 \\
\midrule
Rnd. 2 & LLM$_\text{RJS}$-v2 & LLM$_\text{RJS}$-v1 & {RM$_\text{Base}$} & 2e-6 &    1.896 & 1.551 \\
Rnd. 2 & LLM$_\text{APO}$-v2 &  LLM$_\text{APO}$-v1 &      {RM$_\text{APO}$-v2}      &  2e-6     & 1.975 & 1.586 \\
\midrule
Rnd. 3 & LLM$_\text{RJS}$-v3 & LLM$_\text{RJS}$-v2 & {RM$_\text{Base}$} & 9e-7 &    2.106 & 1.764 \\
Rnd. 3 & LLM$_\text{APO}$-v3 &  LLM$_\text{APO}$-v2 &      {RM$_\text{APO}$-v3}      &  9e-7     &\textbf{2.204} & \textbf{1.807} \\
\bottomrule
\end{tabular}%
}
   
\end{table}

==> tables/rm_results.tex <==
% Table generated by Excel2LaTeX from sheet 'APO_final'
\begin{table}[]
    \centering
    \caption{Training setups and performance of reward models.}
    \label{tab:rm_results}
    \resizebox{\textwidth}{!}{
% Table generated by Excel2LaTeX from sheet 'APO_final'
\begin{tabular}{llllrrrrr}
\toprule
\textbf{Round} & \textbf{Model} & \textbf{Training Data} & \textbf{Base} & \textbf{LR} & \textbf{Helpful} & \textbf{Harmless} & \textbf{H\&H Avg.} &\textbf{Align.Dev.} \\
\midrule
Eval. RM &RM$_\text{Test}$ & H\&H & LLaMA-7B & 1e-6 &  &  &  &  \\
%\hline
 &{RM$_\text{All}$} & H\&H + WebGPT + GPT4LLM & LLaMA-7B & {1e-6} &  \\
\midrule
Round 0 &{RM$_\text{Base}$} & {H\&H$_\text{RM}$} & {LLaMA-7B} &  1e-6     & 63.14 & 62.93 & 63.04 & 68.63 \\

\midrule
Round 1 &RM$_\text{APO}$-v1 & H\&H$_\text{RM}$ + Sample$_\text{APO}$-v0 & {RM$_\text{Base}$} & 1e-7 & 63.95 & 64.40 & 64.17 & 69.97 \\
%\hline
 &{RM$_\text{Base}$-{AB}} & {H\&H$_\text{RM}$} & {RM$_\text{Base}$} & {1e-7} & 63.35 & 63.71 & 63.53 & 68.55 \\
\midrule
Round 2 &{RM$_\text{APO}$-v2} & {H\&H$_\text{RM}$ + Sample$_\text{APO}$-v1} & {RM$_\text{Base}$} & {1e-7} & 63.52 & 64.40 & 63.96 & 70.02 \\
 &{RM$_\text{APO}$-v2seq} & {H\&H$_\text{RM}$ + Sample$_\text{APO}$-v1} & {RM$_\text{APO}$-v1} & {1e-7} & 63.52 & 63.71 & 63.62 & 70.37 \\
\midrule
Round 3 &{RM$_\text{APO}$-v3} & {H\&H$_\text{RM}$ + Sample$_\text{APO}$-v2} & {RM$_\text{Base}$} & {1e-7} & 63.77 & 64.31 & 64.04 & 69.70 \\
 &{RM$_\text{APO}$-v3seq} & {H\&H$_\text{RM}$ + Sample$_\text{APO}$-v2} & {RM$_\text{APO}$-v2seq} & {1e-7} & 63.77 & 64.70 & 64.24 & 70.13 \\
\bottomrule
\end{tabular}%

}
\end{table}

==> tables/rm_results_1110.tex <==
% Table generated by Excel2LaTeX from sheet 'APO_final'
\begin{table*}[t]
    \centering
    \caption{Training setups and performance of reward models.}
    \label{tab:rm_results}
    \vspace{-1mm}
    \resizebox{0.999\textwidth}{!}{
% Table generated by Excel2LaTeX from sheet 'APO_final'
\begin{tabular}{llllrrrrr}
\toprule
\textbf{Round} & \textbf{Model} & \textbf{Training Data} & \textbf{Base} & \textbf{Test Acc} & \textbf{Test ECE} & \textbf{Dev Acc}& \textbf{Dev ECE} \\
\midrule
Eval.  &{RM$_\text{All}$} & HH + WebGPT + GPT4LLM & LLaMA-7B & 72.98 & 0.011 & 76.51 &0.029 \\
 &RM$_\text{Test}$ & HH & LLaMA-7B & 72.34  & 0.010  & 75.69 & 0.025  \\
\midrule
Rnd. 0 &{RM$_\text{Base}$} & {HH$_\text{RM}$} & {LLaMA-7B} &  63.04 & 0.019 & 63.18 & 0.014 \\

\midrule
Rnd. 1 &RM$_\text{APO}$-v1 & HH$_\text{RM}$ + Sample$_\text{APO}$-v0 & {RM$_\text{Base}$}  & 64.17 & 0.064 & 64.59 & 0.058 \\
%\hline
 &{RM$_\text{Base}$-{AB}} & {HH$_\text{RM}$} & {RM$_\text{Base}$} & 63.53 & 0.046 & 63.55 & 0.043 \\
\midrule
Rnd. 2 &{RM$_\text{APO}$-v2} & {HH$_\text{RM}$ + Sample$_\text{APO}$-v1} & {RM$_\text{Base}$} & 63.95 & 0.067 & 64.38 & 0.060 \\
 &{RM$_\text{APO}$-v2seq} & {HH$_\text{RM}$ + Sample$_\text{APO}$-v1} & {RM$_\text{APO}$-v1} & 63.61 & 0.091 & 64.93 & 0.075 \\
\midrule
Rnd. 3 &{RM$_\text{APO}$-v3} & {HH$_\text{RM}$ + Sample$_\text{APO}$-v2} & {RM$_\text{Base}$}  & 64.04 & 0.067 & 64.27 & 0.062 \\
 &{RM$_\text{APO}$-v3seq} & {HH$_\text{RM}$ + Sample$_\text{APO}$-v2} & {RM$_\text{APO}$-v2seq}  & 64.23 & 0.104 & 65.02 & 0.093 \\
\bottomrule
\end{tabular}%

}
\end{table*}

==> tables/rm_results_no_seq.tex <==
% Table generated by Excel2LaTeX from sheet 'APO_final'
\begin{table}[t]
    \centering
    \caption{Training setups and performance of reward models.}
    \label{tab:rm_results}
    \vspace{-1mm}
    \resizebox{0.999\textwidth}{!}{
% Table generated by Excel2LaTeX from sheet 'APO_final'
\begin{tabular}{llllrrr}
\toprule
\textbf{Round} & \textbf{Model} & \textbf{Training Data} & \textbf{Base} & \textbf{Test Acc} & \textbf{Dev Acc} \\
\midrule
Eval.  &{RM$_\text{All}$} & HH + WebGPT + GPT4LLM & LLaMA-7B & 72.98 &  76.51 \\
 &RM$_\text{Test}$ & HH & LLaMA-7B & 72.34   & 75.69   \\
\midrule
Rnd. 0 &{RM$_\text{Base}$} & {HH$_\text{RM}$} & {LLaMA-7B} &  63.04 & 63.18 \\

\midrule
Rnd. 1 &RM$_\text{APO}$-v1 & HH$_\text{RM}$ + Sample$_\text{APO}$-v0 & {RM$_\text{Base}$}  & 64.17  & 64.59  \\
%\hline
 &{RM$_\text{Base}$-{AB}} & {HH$_\text{RM}$} & {RM$_\text{Base}$} & 63.53 &  63.55  \\
\midrule
Rnd. 2 &{RM$_\text{APO}$-v2} & {HH$_\text{RM}$ + Sample$_\text{APO}$-v1} & {RM$_\text{Base}$} & 63.95 & 64.38  \\
\midrule
Rnd. 3 &{RM$_\text{APO}$-v3} & {HH$_\text{RM}$ + Sample$_\text{APO}$-v2} & {RM$_\text{Base}$}  & 64.04 &  64.27 \\
\bottomrule
\end{tabular}%
}
\end{table}
